Dualizing sup-preserving endomaps of a complete lattice

It is argued in (Eklund et al., 2018) that the quantale [L,L] of sup-preserving endomaps of a complete lattice L is a Girard quantale exactly when L is completely distributive. We have argued in (Santocanale, 2020) that this Girard quantale structure arises from the dual quantale of inf-preserving endomaps of L via Raney's transforms and extends to a Girard quantaloid structure on the full subcategory of SLatt (the category of complete lattices and sup-preserving maps) whose objects are the completely distributive lattices. It is the goal of this talk to illustrate further this connection between the quantale structure, Raney's transforms, and complete distributivity. Raney's transforms are indeed mix maps in the isomix category SLatt and most of the theory can be developed relying on naturality of these maps. We complete then the remarks on cyclic elements of [L,L] developed in (Santocanale, 2020) by investigating its dualizing elements. We argue that if [L,L] has the structure a Frobenius quantale, that is, if it has a dualizing element, not necessarily a cyclic one, then L is once more completely distributive. It follows then from a general statement on involutive residuated lattices that there is a bijection between dualizing elements of [L,L] and automorphisms of L. Finally, we also argue that if L is finite and [L,L] is autodual, then L is distributive.

==> eptcsdata.tex <==
\providecommand{\firstpage}{335}
\providecommand{\publicationstatus}{David I. Spivak and Jamie Vicary (Eds.):\\
Applied Category Theory 2020 (ACT2020)\\
EPTCS 333, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.333.23}{10.4204/EPTCS.333.23}}


==> macros.tex <==
\RequirePackage{xspace}
\RequirePackage{mytheorems}
\RequirePackage{textlogic}
\RequirePackage{color}
\RequirePackage{tikz-cd}
\RequirePackage{enumerate}
\RequirePackage{paralist}

\RequirePackage{comment}
\excludecomment{proofExtended}
\excludecomment{shortened}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{#1}
\newcommand{\BOF}{\red{BOOF ???}}

\newcommand{\intfun}{\,\cdot\,}
\newcommand{\fun}[1]{(\intfun)^{#1}}
\newcommand{\FUN}{(\intfun)}

\newcommand{\meetof}[1]{{#1}{}^{\land}}
\newcommand{\joinof}[1]{{#1}{}^{\vee}}
\newcommand{\jm}[1]{\meetof{#1}\joinof{}}
\newcommand{\funJoinOf}{\fun{\vee}}
\newcommand{\funMeetOf}{\fun{\land}}
\newcommand{\MEETOF}{\funMeetOf}
\newcommand{\JOINOF}{\funJoinOf}
\newcommand{\DUAL}{\fun{\partial}}
\newcommand{\dual}[1]{#1^{\partial}}
\newcommand{\STAR}{\fun{\star}}
\newcommand{\Star}[2][\ast]{#2{}^{#1}}
\newcommand{\Perp}[2][\perp]{{}^{#1}#2}
\newcommand{\Starf}[1]{\Star{f}(#1)}
\newcommand{\Perpf}[1]{\meetof{f}(#1)}
\newcommand{\EL}{\HomJ{L,L}}
\newcommand{\HLM}{\HomJ{L,M}}
\newcommand{\HXY}{\HomJ{X,Y}}
\newcommand{\HRXY}{\HomR{X,Y}}
\newcommand{\HMXY}{\HomM{X,Y}}
\newcommand{\HMYX}{\HomM{Y,X}}

\newif\ifAbstract
\Abstractfalse

\newcommand{\mc}{inf-preserving\xspace}
\ifx\Mc\undefined
\newcommand{\Mc}{Inf-preserving\xspace}
\else
\renewcommand{\Mc}{Inf-preserving\xspace}
\fi
\newcommand{\jc}{sup-preserving\xspace}
\newcommand{\meets}{infs\xspace}
\newcommand{\joins}{sups\xspace}


\newcommand{\contr}{contradiction\xspace}
\newcommand{\cjp}{completely join-prime\xspace}
\newcommand{\cjirr}{completely join-irreducible\xspace}
\newcommand{\cmirr}{completely meet-irreducible\xspace}
\newcommand{\cmp}{completely meet-prime\xspace}
\newcommand{\rto}[1][\;]{\xrightarrow{\;\;#1\;\;}}
\newcommand{\ddownarrow}{\,\downarrow\!\!\downarrow}
\newcommand{\eqdef}{:=}
\newcommand{\ra}[1]{\rho(#1)}
\newcommand{\la}[1]{\ell(#1)}
\newcommand{\radj}{right adjoint\xspace}
\newcommand{\ladj}{left adjoint\xspace}

\newcommand{\set}[1]{\{ \,#1\, \}}

\newcommand{\Q}{{\mathcal{Q}}} 
\newcommand{\D}{{\mathcal{D}}} 
\newcommand{\QD}{\Q(D)} 
\newcommand{\DP}[1][P]{\D(#1)} 
\newcommand{\QDP}{\Q(\D(P))} 
\newcommand{\QL}{\Q(L)} 
\newcommand{\QC}{\Q(C)} 
\newcommand{\C}{{\mathcal{C}}} 
\newcommand{\R}{{\mathbb{R}}} 

\newcommand{\SL}{\textsf{SLatt}\xspace}
\newcommand{\SLatt}{\SL} 
\newcommand{\CDLatt}{\text{Cd-\SLatt}\xspace} 
\newcommand{\MLatt}{\ensuremath{\mathsf{Latt}_{\bigwedge}}\xspace} 

\newcommand{\iq}{involutive quantaloid\xspace}
\newcommand{\Iq}{Involutive quantaloid\xspace}
\newcommand{\iqe}{involutive quantale\xspace}
\newcommand{\qe}{quantale\xspace}
\newcommand{\rl}{residuated lattice\xspace}
\newcommand{\irl}{involutive \rl}
\newcommand{\upon}{/}
\newcommand{\below}{\backslash}

\RequirePackage{tikz}
\tikzset{
    labl/.style={rotate=90}
}

\newcommand{\commTriangle}[6]{
  \begin{tikzcd}[ampersand replacement=\&]
    #1 \ar[rd, "#4"] \ar[rr, "#6"]\& {} \& #3 \\
    \& #2 \ar[ru, "#5"]\ar[phantom, u, "\leq" labl] \&
  \end{tikzcd}
}

\newcommand{\cjh}{complete join-homomorphism\xspace} 
\newcommand{\cond}[2]{#1 < #2} 
\newcommand{\Cond}[2]{#2 \not\leq #1} 
\newcommand{\COND}[2]{#1 \not\leq #2} 
\newcommand{\fantastic}{fantastic\xspace} 
\newcommand{\jfantastic}{join-\fantastic} 
\newcommand{\mfantastic}{meet-\fantastic} 
\renewcommand{\int}{\mathtt{int}}
\newcommand{\cl}{\mathtt{cl}}
\newcommand{\clatt}{complete lattice\xspace}
\newcommand{\cc}{complete chain\xspace}
\newcommand{\cdlatt}{\cd lattice\xspace}
\newcommand{\Cdlatt}{\Cd lattice\xspace}
\newcommand{\twocomp}{$2$-compatible\xspace}
\newcommand{\cd}{completely distributive\xspace}
\newcommand{\cdity}{complete distributivity\xspace}
\newcommand{\Cdity}{Complete distributivity\xspace}
\newcommand{\Cd}{Completely distributive\xspace}
\newcommand{\bigWedge}{\bigwedge\!\!\!\!\!\!\!\bigwedge}
\newcommand{\sg}{semigroup\xspace}

\renewcommand{\tiff}{\text{iff}\xspace}
\newcommand{\Tiff}{\;\;\tiff\;\;}

\newenvironment{thm}{\vskip 6pt\par\noindent{\bf Theorem.~}\em}{\par\vskip 6pt}
\newenvironment{prop}[1]{\vskip 6pt\par\noindent{\bf Proposition~#1.~}\em}{\par\vskip 6pt} 
\newenvironment{cor}{\vskip 6pt\par\noindent{\bf Corollary.~}\em}{\par\vskip 6pt}

\newcommand{\propno}{2.6.18\xspace}



\newcommand{\tensor}{\otimes}
\newcommand{\jcf}{\jc function\xspace}
\newcommand{\mcf}{\mc function\xspace}


\newcommand{\jirr}{join-irreducible\xspace}
\newcommand{\mirr}{meet-irreducible\xspace}
\newcommand{\jpr}{join-prime\xspace}
\newcommand{\mpr}{meet-prime\xspace}
\newcommand{\je}{join-endomorphism\xspace}
\newcommand{\op}{order-preserving\xspace}
\newcommand{\covers}{\lhd}

\newcommand{\End}{End}
\newcommand{\J}{\mathsf{J}}
\newcommand{\M}{\mathsf{M}}
\newcommand{\JL}{\J(L)}
\newcommand{\ML}{\M(L)}

\newcommand{\shortRHS}[2][15mm]{\makebox[#1][l]{${\displaystyle{#2}}$}}
\newcommand{\TODO}{\textcolor{red}{TODO}}
\newcommand{\interior}[1]{\joinof{\meetof{#1}}}

\newcommand{\Hom}[1]{[#1]}
\newcommand{\HomR}[1]{\HomJ{#1}^{\mathtt{t}}}
\newcommand{\HomM}[1]{\Hom{#1}_{\land}}
\newcommand{\HomJ}[1]{\Hom{#1}_{\vee}}

\newcommand{\Rf}{Raney's function\xspace}
\newcommand{\cjsl}{complete join-semilattice\xspace}
\newcommand{\boxTensor}{\,\Box\,}

\newcommand{\mix}{\ensuremath{\mathsf{mix}}}
\newcommand{\isomix}{isomix\xspace}

\newcommand{\et}{elementary tensor\xspace}
\newcommand{\dset}{\downarrow}
\newcommand{\eExample}{\hfill\ensuremath{\Diamond}}
\newcommand{\EndOfExample}{\eExample}


\newcommand{\Gq}{Girard quantale\xspace}
\newcommand{\Fq}{Frobenius quantale\xspace}
\newcommand{\Gqoid}{Girard quantaloid\xspace}
\newcommand{\saut}{$\ast$-autonomous\xspace}

\newcommand{\two}{\ensuremath{\mathbf{2}}}
\newcommand{\iso}{\simeq}

\newcommand{\upTensor}{\overline{\tensor}}
\newcommand{\doTensor}{\underline{\tensor}}

\newcommand{\END}{\end{document}}
\newcommand{\bimorphism}{bimorphism\xspace}

\newcommand{\Impl}{\ensuremath{\Rightarrow}\xspace}
\newcommand{\Equiv}{\ensuremath{\Leftrightarrow}}
\newcommand{\stepImpl}[2]{(#1) \Impl (#2).~}
\newcommand{\stepEquiv}[2]{$(#1) \Equiv (#2):$~}
\newcommand{\adj}{\dashv}

\newcommand{\HLL}{\HomJ{L,L}}
\newcommand{\HRLL}{\HomR{L,L}}
\newcommand{\Rt}{Raney's transform\xspace}
\newcommand{\RT}{Raney's Theorem\xspace}

\newcommand{\card}[1]{|#1|}
\renewcommand{\paragraph}[1]{\medskip\par\noindent{\bf #1}~}


\newcommand{\CSMC}{closed symmetric monoidal category\xspace}
\newcommand{\SMC}{symmetric monoidal closed\xspace}


